Multiplicity and net-electric charge fluctuations in central Ar+Sc interactions at 13A, 19A, 30A, 40A, 75A, and 150A GeV/c beam momenta measured by NA61/SHINE at the CERN SPS

This paper presents results on multiplicity fluctuations of positively and negatively charged hadrons as well as net-electric charge fluctuations measured in central Ar+Sc interactions at beam momenta 13A, 19A, 30A, 40A, 75A, and 150A GeV/c. The fluctuation analysis is one of the tools to search for the predicted critical point of strongly interacting matter. Results are corrected for the experimental biases and quantified using cumulant ratios. In most instances, multiplicity and net-charge distributions appear narrower than the corresponding Poisson or Skellam distributions. Cumulant ratios are compared with the EPOS1.99 model predictions, which provide a qualitative description that aligns with observations for positively and negatively charged particles. The obtained results are also compared to earlier NA61/SHINE results from inelastic p+p interactions in the same analysis acceptance.

==> na61Abbreviations.tex <==
%%%%%%% units
\newcommand{\kg}{\ensuremath{\mbox{kg}}\xspace}
\newcommand{\eV}{\ensuremath{\mbox{e\kern-0.1em V}}\xspace}
\newcommand{\GeV}{\ensuremath{\mbox{Ge\kern-0.1em V}}\xspace}
\newcommand{\MeV}{\ensuremath{\mbox{Me\kern-0.1em V}}\xspace}
\newcommand{\GeVc}{\ensuremath{\mbox{Ge\kern-0.1em V}\!/\!c}\xspace}
\newcommand{\GeVcc}{\ensuremath{\mbox{Ge\kern-0.1em V}\!/\!c^2}\xspace}
\newcommand{\AGeV}{\ensuremath{A\,\mbox{Ge\kern-0.1em V}}\xspace}
\newcommand{\AGeVc}{\ensuremath{A\,\mbox{Ge\kern-0.1em V}\!/\!c}\xspace}
\newcommand{\MeVc}{\ensuremath{\mbox{Me\kern-0.1em V}/c}\xspace}
\newcommand{\T}{\ensuremath{\mbox{T}}\xspace}
\newcommand{\cmsq}{\ensuremath{\mbox{cm}^2}\xspace}
\newcommand{\msq}{\ensuremath{\mbox{m}^2}\xspace}
\newcommand{\cm}{\ensuremath{\mbox{cm}}\xspace}
\newcommand{\mm}{\ensuremath{\mbox{mm}}\xspace}
\newcommand{\micron}{\ensuremath{\mu\mbox{m}}\xspace}
\newcommand{\mrad}{\ensuremath{\mbox{mrad}}\xspace}
\newcommand{\ns}{\ensuremath{\mbox{ns}}\xspace}
\newcommand{\m}{\ensuremath{\mbox{m}}\xspace}
\newcommand{\s}{\ensuremath{\mbox{s}}\xspace}
\newcommand{\ms}{\ensuremath{\mbox{ms}}\xspace}
\newcommand{\ps}{\ensuremath{\mbox{ps}}\xspace}
\newcommand{\dd}{\ensuremath{{\text{d}}}\xspace}
\newcommand{\dedx}{\ensuremath{\dd E\!/\!\dd x}\xspace}
\newcommand{\tof}{\ensuremath{\textup{\emph{tof}}}\xspace}
\newcommand{\pt}{\ensuremath{p_{\text{T}}}\xspace}
\newcommand{\PT}{\ensuremath{P_\textup{T}}\xspace}
\newcommand{\mt}{\ensuremath{m_{\text{T}}}\xspace}

%particles
\newcommand{\pbar}{\ensuremath{\overline{p}}\xspace}
\newcommand{\pim}{\ensuremath{\pi^-}\xspace}
\newcommand{\pip}{\ensuremath{\pi^+}\xspace}
\newcommand{\km}{\ensuremath{K^-}\xspace}
\newcommand{\kp}{\ensuremath{K^+}\xspace}
\newcommand{\hm}{\ensuremath{h^-}\xspace}
\newcommand{\pp}{\mbox{\textit{p+p}}\xspace}
\newcommand{\pA}{\mbox{\textit{p}+A}\xspace}

\newcommand{\W}{$\langle W\rangle$}
\newcommand{\piMin}{$\langle \pi^-\rangle$ }
\newcommand{\dEdx}{$\text{d}E/\text{d}x$ }
\newcommand{\dydpt}{$dydp_T$ }
\newcommand{\coordinate}[1]{{\fontfamily{lmss}\selectfont#1}}




% inverse hyperbolic functions
%\DeclareMathOperator{\acosh}{acosh}
%\DeclareMathOperator{\asinh}{asinh}
%\DeclareMathOperator{\atanh}{atanh}

%%%%%%%%%%%%% some software programs and generators
%----- NA61 software
\def\Offline{\mbox{$\overline{\text%
{Off}}$\hspace{.05em}\raisebox{.4ex}{\underline{line}}}\xspace}
\def\SHOE{\mbox{SHO\hspace{-1.34ex}\raisebox{0.2ex}{\color{green}\textasteriskcentered}\hspace{0.25ex}E}\xspace}
\def\DSHACK{\mbox{DS\hspace{0.15ex}$\hbar$ACK}\xspace}
\DeclareRobustCommand{\SHINE}{\mbox{\textsc{S\hspace{.05em}\raisebox{.4ex}{\underline{hine}}}}\xspace} %DeclareRobustCommand allows this to work in caption
%\def\SHINE{\textsc{Shine}\xspace}
%----- event generators
\def\Glissando{\textsc{Glissando}\xspace}
\newcommand{\Smash}{{\scshape Smash}\xspace}
\newcommand{\SmashLong}{{\scshape Smash1.5}\xspace}
\newcommand{\FlukaLong}{{\scshape Fluka2008}\xspace}
\newcommand{\FlukaEleven}{{\scshape Fluka2011}\xspace}
\newcommand{\Fluka}{{\scshape Fluka}\xspace}
\newcommand{\UrqmdLong}{{\scshape U}r{\scshape qmd1.3.1}\xspace}
\newcommand{\Urqmd}{{\scshape U}r{\scshape qmd}\xspace}
\newcommand{\GheishaLong}{{\scshape Gheisha2002}\xspace}
\newcommand{\GheishaOld}{{\scshape Gheisha600}\xspace}
\newcommand{\Gheisha}{{\scshape Gheisha}\xspace}
\newcommand{\Corsika}{{\scshape Corsika}\xspace}
\newcommand{\Venus}{{\scshape Venus}\xspace}
\newcommand{\VenusLong}{{\scshape Venus4.12}\xspace}
\newcommand{\GiBUU}{{\scshape GiBUU}\xspace}
\newcommand{\GiBUULong}{{\scshape GiBUU1.6}\xspace}
\newcommand{\FlukaNewLong}{{\scshape Fluka2011.2\_17}\xspace}
\newcommand{\Root}{{\scshape Root}\xspace}
\newcommand{\Geant}{{\scshape Geant}\xspace}
\newcommand{\GeantThree}{{\scshape Geant3}\xspace}
\newcommand{\GeantFour}{{\scshape Geant4}\xspace}
\newcommand{\QGSJet}{{\scshape QGSJet}\xspace}
\newcommand{\DPMJet}{{\scshape DPMJet}\xspace}
\newcommand{\Epos}{{\scshape Epos}\xspace}
\newcommand{\EposLong}{{\scshape Epos1.99}\xspace}
\newcommand{\QGSJetLong}{{\scshape QGSJetII-04}\xspace}
\newcommand{\DPMJetLong}{{\scshape DPMJet3.06}\xspace}
\newcommand{\SibyllLong}{{\scshape Sibyll2.1}\xspace}
\newcommand{\EposLHCLong}{{\scshape EposLHC}\xspace}
\newcommand{\Hsd}{{\scshape Hsd}\xspace}
\newcommand{\Ampt}{{\scshape Ampt}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%% misc
\def\red#1{{\color{red}#1}}
\def\avg#1{\langle{#1}\rangle}
\def\sci#1#2{#1\!\times\!10^{#2}}
\newcommand{\Fi}[1]{Fig.~\ref{#1}}
\newcommand{\CernVM}{\textsc{Cern\-\kern-0.05emVM}\xspace}


==> na61AuthorsLimited.tex <==
% based on XML DB with time Wed Oct 30 22:28:26 2024
% Authors in alphabetical order.

\noindent
{T.\;Anti\'ci\'c~\href{https://orcid.org/0000-0002-6606-0191}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,1}},
{S.\;Bordoni\textsuperscript{\,7}},
{A.\;Bravar\textsuperscript{\,6}},
{N.\;Charitonidis\textsuperscript{\,7}},
{G.\;Christodoulou\textsuperscript{\,7}},
{A.\;De~Roeck\textsuperscript{\,7}},
{F.\;Diakonos\textsuperscript{\,2}},
{S.J.\;Dolan\textsuperscript{\,7}},
{R.A.\;Fernandez\textsuperscript{\,7}},
{K.J.\;Floethner\textsuperscript{\,7}},
{A.\;Kapoyannis\textsuperscript{\,2}},
{U.\;Kose\textsuperscript{\,7}},
{M.O.\;Kuttan\textsuperscript{\,3}},
{O.\;Linnyk\textsuperscript{\,3}},
{L.\;Munteanu\textsuperscript{\,7}},
{C.\;Mussolini\textsuperscript{\,7}},
{J.\;Pawlowski\textsuperscript{\,3}},
{W.\;Rauch\textsuperscript{\,4}},
{L.\;Scharenberg\textsuperscript{\,7}},
{S.\;Schramm\textsuperscript{\,3}},
{J.\;Steinheimer-Froschauer\textsuperscript{\,3}},
{H.\;Stoecker\textsuperscript{\,3}},
{H.\;Str\"obele\textsuperscript{\,5}},
{T.\;\v{S}u\v{s}a~\href{https://orcid.org/0000-0001-7430-2552}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,1}},
{A.\;Toia~\href{https://orcid.org/0000-0001-9567-3360}{\includegraphics[height=1.7ex]{orcid-logo.png}}\textsuperscript{\,5}},
{M.\;Vassiliou\textsuperscript{\,2}},
{C.F.\;Vilela\textsuperscript{\,7}}, and
{K.\;Zhou\textsuperscript{\,3}}


==> na61InstitutionsLimited.tex <==
% based on XML DB with time Wed Oct 30 22:28:26 2024
% Institutes in alphabetical order.

\noindent
\textsuperscript{1}~Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia\\
\textsuperscript{2}~University of Athens, Athens, Greece\\
\textsuperscript{3}~Frankfurt Institute for Advanced Studies, Frankfurt, Germany\\
\textsuperscript{4}~Fachhochschule Frankfurt, Frankfurt, Germany\\
\textsuperscript{5}~University of Frankfurt, Frankfurt, Germany\\
\textsuperscript{6}~University of Geneva, Geneva, Switzerland\\
\textsuperscript{7}~CERN, Geneva, Switzerland\\

